On the Neural Tangent Kernel Analysis of Randomly Pruned Neural Networks

Motivated by both theory and practice, we study how random pruning of the weights affects a neural network's neural tangent kernel (NTK). In particular, this work establishes an equivalence of the NTKs between a fully-connected neural network and its randomly pruned version. The equivalence is established under two cases. The first main result studies the infinite-width asymptotic. It is shown that given a pruning probability, for fully-connected neural networks with the weights randomly pruned at the initialization, as the width of each layer grows to infinity sequentially, the NTK of the pruned neural network converges to the limiting NTK of the original network with some extra scaling. If the network weights are rescaled appropriately after pruning, this extra scaling can be removed. The second main result considers the finite-width case. It is shown that to ensure the NTK's closeness to the limit, the dependence of width on the sparsity parameter is asymptotically linear, as the NTK's gap to its limit goes down to zero. Moreover, if the pruning probability is set to zero (i.e., no pruning), the bound on the required width matches the bound for fully-connected neural networks in previous works up to logarithmic factors. The proof of this result requires developing a novel analysis of a network structure which we called \textit{mask-induced pseudo-networks}. Experiments are provided to evaluate our results.

==> wrong_stuff.tex <==
\begin{lemma}
\textcolor{red}{Wrong way of doing things: no concentration}
Let $\mathbf{v} \in \R^n$ and $\mathbf{m} \in \R^n$ where $\mathbf{m}_i \sim \frac{1}{\sqrt{\alpha}} \textnormal{Bernoulli}(\alpha)$. 
Then, with probability $1 - \delta$,
\begin{align*}
    \norm{\mathbf{v} \odot \mathbf{m}}_2^2 \lesssim
\end{align*}
\end{lemma}
\begin{proof}
First of all, we have $\E[\norm{\mathbf{v} \odot \mathbf{m}}_2^2] = \norm{\mathbf{v}}_2^2$.
Then, 
\begin{align*}
    \mathbf{m}_i^2 & \sim \textnormal{subgamma}\left( 4+4\left( \frac{1 - \alpha}{\alpha} \right)^2, 2 \frac{1 - \alpha}{\alpha} \right) \\
    \Rightarrow \mathbf{v}_i^2 \mathbf{m}_i^2 &\sim \textnormal{subgamma}\left( \mathbf{v}_i^4 \left(4 + \left( \frac{1 - \alpha}{\alpha} \right)^2 \right), 2 \mathbf{v}_i^2 \frac{1 - \alpha}{\alpha} \right) \\
    \Rightarrow \norm{\mathbf{v} \odot \mathbf{m}}_2^2 &\sim \textnormal{subgamma}\left( \norm{\mathbf{v}}_2^4 \left(4 + \left( \frac{1 - \alpha}{\alpha} \right)^2 \right), 2\norm{\mathbf{v}}_2^2 \frac{1 - \alpha}{\alpha} \right)
\end{align*}
Thus, with probability $1 - \delta$, 
\begin{align*}
    \norm{\mathbf{v} \odot \mathbf{m}}_2^2 \lesssim \norm{\mathbf{v}}_2^2 + \sqrt{\norm{\mathbf{v}}_2^4 \left(4 + \left( \frac{1 - \alpha}{\alpha} \right)^2 \right) \log \frac{1}{\delta}} + 2\norm{\mathbf{v}}_2^2 \frac{1 - \alpha}{\alpha} \log \frac{1}{\delta}
\end{align*}
\end{proof}


\textcolor{red}{Think about taking out $\mathbf{m}_j$. 
We apply leave-one-out analysis and analyze that the dependence part is small and independent part is also small as well. }
Let's us do some wishful thinking. 
Suppose $\mathbf{m}_{ij}^{(h+1)} \mathbf{g}_j^{(h)}$ is indeed independent of the rest. 
Then take the expectation over $\mathbf{m}_{ij}^{(h+1)}$ will give us $\mathbf{g}_j^{(h)}$ on the diagonal. 
Define 
\begin{align*}
   \tilde{\mathbf{f}}^{(h+1)} = 
   \begin{bmatrix}
    \left( {\mathbf{w}}^{(h+1)}_{1, \backslash j} \odot \mathbf{m}^{(h+1)}_{1, \backslash j} \right)^\top \mathbf{g}^{(h)}_{\backslash j} \\
    \left( {\mathbf{w}}^{(h+1)}_{2, \backslash j} \odot \mathbf{m}^{(h+1)}_{2, \backslash j} \right)^\top \mathbf{g}^{(h)}_{\backslash j} \\
    \vdots \\
    \left( {\mathbf{w}}^{(h+1)}_{d_{h+1}, \backslash j} \odot \mathbf{m}^{(h+1)}_{d_{h+1}, \backslash j} \right)^\top \mathbf{g}^{(h)}_{\backslash j}
    \end{bmatrix} 
\end{align*}
This gives us
\begin{align*}
    \mathbf{f}^{(h+1)} - \tilde{\mathbf{f}}^{(h+1)} = 
\begin{bmatrix}
    {\mathbf{w}}^{(h+1)}_{1, j}  \mathbf{m}^{(h+1)}_{1, j} \mathbf{g}^{(h)}_{j} \\
    {\mathbf{w}}^{(h+1)}_{2, j} \mathbf{m}^{(h+1)}_{2, j} \mathbf{g}^{(h)}_{j} \\
    \vdots \\
    {\mathbf{w}}^{(h+1)}_{d_{h+1}, j} \mathbf{m}^{(h+1)}_{d_{h+1}, j}  \mathbf{g}^{(h)}_{j}
\end{bmatrix}
\end{align*}
We are going to show that both 
\begin{align}
    & \left| \mathbf{g}_j^{(h)} \left( \mathbf{b}^{(h+1)}(\mathbf{x}^{(1)}) \right)^\top \textnormal{diag}\left(\frac{\frac{1}{\sqrt{\alpha}} \mathbf{m}_{ij}^{(h+1)} }{\norm{\mathbf{g}^{(h)} \odot \mathbf{m}_i^{(h+1)}}_2^2} \right) \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) \right| \label{eqn: independent_term}\\
    & \left|\mathbf{g}_j^{(h)} \left( \mathbf{b}^{(h+1)}(\mathbf{x}^{(1)}) \right)^\top \textnormal{diag}\left(\frac{\frac{1}{\sqrt{\alpha}} \mathbf{m}_{ij}^{(h+1)} }{\norm{\mathbf{g}^{(h)} \odot \mathbf{m}_i^{(h+1)}}_2^2} \right) \left( \mathbf{f}^{(h+1)}(\mathbf{x}^{(1)}) - \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) \right) \right| \label{eqn: dependent_term}
\end{align}
are small.
This can be reduced to derive the expectation and concentration property of 
\begin{align*}
    & \frac{c_\sigma}{d_{h+1}} \norm{\mathbf{D}^{(h+1)} \textnormal{diag}\left(\frac{1}{\sqrt{\alpha}} \mathbf{m}^{(h+1)}_{ij} \right) \left( \mathbf{f}^{(h+1)}(\mathbf{x}^{(1)}) - \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) \right)}_2^2 \\
    & \frac{c_\sigma}{d_{h+1}} \norm{\mathbf{D}^{(h+1)} \textnormal{diag}\left(\frac{1}{\sqrt{\alpha}} \mathbf{m}^{(h+1)}_{ij} \right) \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) }_2^2
\end{align*}
We first bound Equation \eqref{eqn: dependent_term}.
Conditioned on $\mathbf{g}^{(h)}$, observe that for each entry $\mathbf{D}^{(h+1)}_{ii} \mathbf{w}_{i,j}^{(h+1)} \mathbf{m}_{i,j}^{(h+1)} \mathbf{g}_j^{(h)} \frac{1}{\alpha}$ we have
\begin{align*}
\E_{\mathbf{W}^{(h+1)}, \mathbf{m}^{(h+1)}} \left[ \left( \mathbf{D}^{(h+1)}_i \mathbf{w}_{i,j}^{(h+1)} \mathbf{m}_{i,j}^{(h+1)} \mathbf{g}_j^{(h)} \frac{1}{{\alpha}} \right)^2 \right] &= \frac{\left( \mathbf{g}_j^{(h)} \right)^2}{2 \alpha^2 }\\
\Rightarrow \E_{\mathbf{W}^{(h+1)}, \mathbf{m}^{(h+1)}} \left[ \frac{c_\sigma}{d_{h+1}} \norm{\mathbf{D}^{(h+1)} \textnormal{diag}\left(\frac{1}{\sqrt{\alpha}} \mathbf{m}^{(h+1)}_{ij} \mathbf{g}_j^{(h)} \right) \left( \mathbf{f}^{(h+1)}(\mathbf{x}^{(1)}) - \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) \right)}_2^2 \right] &= \frac{\left( \mathbf{g}_j^{(h)} \right)^2}{ \alpha^2 }
\end{align*}
The first equality can be proved by first conditioned on $\mathbf{m}^{(h+1)}$ and apply the same distribution trick and then take the expectation over $\mathbf{m}^{(h+1)}$.
Since conditioned on $\mathbf{m}^{(h+1)}, \mathbf{g}$, $\left( \left( \mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)} \right)^\top \mathbf{g} \right)^2 \dot{\sigma} \left( \left( \mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)} \right)^\top \mathbf{g}' \right)$ has the same distribution as $\left( \left( \mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)} \right)^\top \mathbf{g} \right)^2 \dot{\sigma} \left( \left( \mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)} \right)^\top \mathbf{g} \right)$.
Thus, conditioned on $\mathbf{g}^{(h)}$, we have
\begin{align*}
    & \left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top (\mathbf{g}^{(h)} - \mathbf{g}^{(h)}_{\backslash j}) \right)^2 \dot{\sigma}\left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top \mathbf{g}^{(h)} \right) \\
    &\sim \left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top (\mathbf{g}^{(h)} - \mathbf{g}^{(h)}_{\backslash j}) \right)^2 \dot{\sigma}\left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top \mathbf{g}^{(h)}_{\backslash j} \right) \\
    & \left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top \mathbf{g}^{(h)}_{\backslash j} \right)^2 \dot{\sigma}\left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top \mathbf{g}^{(h)} \right) \\
    &\sim \left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top \mathbf{g}^{(h)}_{\backslash j} \right)^2 \dot{\sigma}\left( (\mathbf{w}^{(h+1)} \odot \mathbf{m}^{(h+1)})^\top \mathbf{g}^{(h)}_{\backslash j} \right)
\end{align*}
Next we analyze its concentration property. 
If we fix $\mathbf{g}^{(h)}$ and let $\mathbf{W}^{(h+1)}, \mathbf{m}^{(h+1)}$ vary, then the random variable \textcolor{red}{TODO: Check this.}
\begin{align*}
\left( \mathbf{D}^{(h+1)}_i \mathbf{w}_{i,j}^{(h+1)} \mathbf{m}_{i,j}^{(h+1)} \mathbf{g}_j^{(h)} \frac{1}{{\alpha}} \right)^2 &\sim \textnormal{subgamma}\left( O\left(\frac{1}{\alpha^2} \frac{\left(\mathbf{g}_j^{(h)} \right)^4}{\alpha^4} \right), O\left( \frac{1}{\alpha} \frac{\left(\mathbf{g}_j^{(h)} \right)^2}{\alpha^2} \right) \right) 
\end{align*}
% \begin{align*}
% & \Rightarrow {\frac{c_\sigma}{d_{h+1}}} \norm{\mathbf{D}^{(h+1)} \textnormal{diag}\left(\frac{1}{\sqrt{\alpha}} \mathbf{m}^{(h+1)}_{ij} \right) \left( \mathbf{f}^{(h+1)}(\mathbf{x}^{(1)}) - \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) \right)}_2^2 \\
% &\sim \textnormal{subgamma}\left( O\left(\sum_i \left(\mathbf{m}_{i,j}^{(h+1)} \mathbf{g}_j^{(h)} \right)^8 \frac{1}{d_{h+1}^2 \alpha^2} \right), O\left(\left( \mathbf{g}_j^{(h)} \right)^4 \frac{1}{d_{h+1} \alpha^3} \right) \right) \\
% &= \textnormal{subgamma}\left( O\left( \frac{\left( \mathbf{g}_j^{(h)} \right)^8 }{d_{h+1} \alpha^5} \frac{1}{d_{h+1}} \sum_i \left(\mathbf{m}_{i,j}^{(h+1)} \right)^2 \right), O\left( \frac{\left( \mathbf{g}_j^{(h)} \right)^4}{d_{h+1} \alpha^3} \right) \right)
% \end{align*}
% If $d_{h+1} \gtrsim \left( \frac{1-\alpha}{\alpha} \right)^2 \log \frac{1}{\delta}$ with probability $1 - \delta$, we have $\frac{1}{d_{h+1}} \sum_i \left( \mathbf{m}_{ij}^{(h+1)} \right)^2 \leq 2$. Thus, with probability $1 - \delta$, 
% \begin{align*}
%     & {\frac{c_\sigma}{d_{h+1}}} \norm{\mathbf{D}^{(h+1)} \textnormal{diag}\left(\frac{1}{\sqrt{\alpha}} \mathbf{m}^{(h+1)}_{ij} \mathbf{g}_j^{(h)} \right) \left( \mathbf{f}^{(h+1)}(\mathbf{x}^{(1)}) - \tilde{\mathbf{f}}^{(h+1)}(\mathbf{x}^{(1)}) \right)}_2^2 \\
%     &\lesssim \frac{\left( \mathbf{g}_j^{(h)} \right)^4}{\alpha^2} + \sqrt{ \frac{\left( \mathbf{g}_j^{(h)} \right)^8 }{d_{h+1} \alpha^5} \log \frac{1}{\delta}} + \frac{\left( \mathbf{g}_j^{(h)} \right)^4}{d_{h+1} \alpha^3} \log \frac{1}{\delta} \\
%     &\lesssim \frac{\left( \mathbf{g}_j^{(h)} \right)^4}{\alpha^2} + \frac{\left( \mathbf{g}_j^{(h)} \right)^4}{d_{h+1} \alpha^3} \log \frac{1}{\delta} \\
%     &\lesssim \frac{\left( \mathbf{g}_j^{(h)} \right)^4}{\alpha^2}
% \end{align*}
Next we bound Equation \eqref{eqn: independent_term}.


\textcolor{red}{Consider analyze this for unit norm vectors and then scale the vector.}

